Continuous Tasks and the Chromatic Simplicial Approximation Theorem

The celebrated 1999 Asynchronous Computability Theorem (ACT) of Herlihy and Shavit characterized the distributed tasks that are wait-free solvable, and thus uncovered a deep connection with algebraic topology. We present a novel interpretation of this theorem, through the notion of continuous task, defined by an input/output specification that is a continuous function. To do so, we introduce a chromatic version of a foundational result for algebraic topology: the simplicial approximation theorem. In addition to providing a different proof of the ACT, the notion of continuous task seems interesting in itself. Indeed, besides the fact that certain distributed problems are naturally specified by continuous functions, continuous tasks have an expressive power that also allows to specify the density of desired outputs for each combination of possible inputs,for example.

==> preliminaries.tex <==
% !TEX root = main.tex
\section{Preliminaries}

In the first subsection we describe the model and other notions from distributed computing. In the 
second subsection, we recall some basic topology notions.
[[[working...]]]
\subsection{Distributed computing}

We consider a set of $n+1$ sequential processes that communicate by reading and writing a shared memory. 
There are many variants of the read/write memory model, but they are computationally equivalent~\cite{HKR13}. For the purposes of this paper and following the ACT presentation~\cite{HS99:ACT}, it is sufficient to say that
we consider any of the variants in which the protocol complex is a chromatic subdivision.
We define these notions below.

Processes are \emph{asynchronous}: there is no bound on relative process speed. Processes can  fail by halting. One process cannot determine whether an unresponsive process has failed or is just slow.
A \emph{task} is a coordination problem in which each process starts with a private input value taken from a finite set, communicates with the other processes, and eventually halts with a private output value, also taken from a finite set. 
A \emph{protocol} is a distributed program that solves a task in a particular model of computation.  A protocol is \emph{wait-free} if it tolerates failures by $n$ out of $n+1$ processes. 


\subsection{Topology}

We begin with some standard basic definitions that can be found in ~\cite{HKR13}. The first definition that we need is the definition of an abstract simplicial complex. An abstract simplicial complex can be thought of as a "high-dimensional" graph. Abstract simplicial complexes have the advantage of having a discrete combinatorial construction, while at the same time, they are able to express triangulated manifolds.

\begin{definition}[Abstract simplicial complex]\label{def:abssimpcomplex}
	An abstract simplicial complex $\mathcal K$ is a pair $\langle V(\mathcal{K}), F(\mathcal{K}) \rangle$, where $V(\mathcal{K})$ is a set, $F(\mathcal{K}) \subseteq 2^{V(\mathcal{K})}$, and for any $\sigma, \tau \in 2^{V(\mathcal{K})}$ such that $\sigma \subseteq \tau$ and  $\tau \in F(\mathcal{K})$, then $\sigma \in F(\mathcal{K})$. $V(\mathcal{K})$ is called the vertex set, and $F(\mathcal{K})$ is the face set of $\mathcal{K}$. The elements of $V(\mathcal{K})$ are called the vertices, and the elements of $F(\mathcal{K})$ are called the faces or simplices. We say that an abstract simplicial complex is \emph{finite} if it's vertex set is finite.
\end{definition}

Intuitively, dimension is a number that represents how many axis we need to describe a point in space. In the following definition we define the dimension of a face or simplex of an abstract simplicial complex.

\begin{definition}[Dimension] \label{def:dimension}
	Let $\mathcal{K}$ be an abstract simplicial complex, and $\sigma \in F(\mathcal{K})$ a simplex. We say that $\sigma$ has dimension $k$, denoted by $\textrm{dim}(\sigma)=k$, if it has a cardinality of $k+1$. We say that $\mathcal{K}$ is of dimension $k$ if it has a simplex of maximum dimension $k$.
\end{definition}

In the context of distributed computing, since local processes' states correspond to vertices, and global configurations correspond to faces, we only consider simplicial complexes where all simplices are of the same dimension. We call this particular type of simplicial complexes \emph{pure abstract simplicial complexes}.

Now that we have defined the basic objects in combinatorial topology, we must also define the morphisms which preserve the structure. 

\begin{definition}[Simplicial maps] \label{def:simpmap}
	Let $\mathcal{K}$ and $\mathcal{L}$ be abstract simplicial complexes. We say that a vertex map $\mu : V(\mathcal{K}) \rightarrow V(\mathcal{L})$ is a simplicial map if for any $\sigma \in F(\mathcal{K}), \mu (\sigma) \in \mathcal{L}$.
\end{definition}

It should be noted that simplicial maps are the discrete analogon to continuous functions. This equivalence is formally stated through the simplicial approximation theorem.

Since we are interested in modeling distributed systems with simplicial complexes, it is usefull to enrich simplicial complexes with a coloring. Such coloring corresponds to extracting the processes' ids from the local states.

\begin{definition}[Coloring]\label{def:coloring}
	Let $\mathcal{K}$ be a finite abstract simplicial complex of dimension $k$. We say that a function $\chi: V(\mathcal{K}) \rightarrow \{1,2, \ldots, k+1\}$ is a proper coloring if for any simplex $\sigma \in F(\mathcal{K})$, $\chi$ is injective at $\sigma$. 
\end{definition}

In order to simplify notation, whenever we have two disjoint abstract simplicial complexes $\mathcal{K}$ and $\mathcal{L}$, both of dimension $k$, with colorings $\mu_1$ and $\mu_2$, we will instead implicitly consider a "global" coloring $\mu: V(\mathcal{K}) \cup V(\mathcal{L}) \rightarrow \{1, \ldots, k+1\}$, since it is simpler and free from ambiguity.

We have now enriched simplicial complex with coloring. Since we are interested that morphisms preserve the structure, then we must also add a coloring restriction.

\begin{definition}[Chromatic simplicial maps]\label{def:chrsimpmap}
	Let $\mathcal{K}$ and $\mathcal{L}$ be abstract simplicial complexes of dimension $k$, and $\chi_1, \chi_2$ proper colorings for $\mathcal{K}$ and $\mathcal{L}$ respectively. We say that a simplicial map is chromatic if for any $v \in V(\mathcal{K}),\; \chi_1(v)) = \chi_2(\mu(v))$.
\end{definition}

\begin{definition}[Subcomplex]
	Let $\mathcal{K}$ and $\mathcal{L}$ be abstract simplicial complexes, we say that $\mathcal{L}$ is a subcomplex of $\mathcal{K}$ if $V(\mathcal{L}) \subseteq V(\mathcal{K})$ and $F(\mathcal{L}) \subseteq F(\mathcal{K})$.
\end{definition}
\begin{definition}\label{def:carrmap}
Let $\mathcal{K}$ and $\mathcal{L}$ be abstract simplicial complexes and $\Phi: \mathcal{K} \rightarrow 2^{\mathcal{L}}$. We say that $\Phi$ is a carrier map if $\Phi(\sigma)$ is a subcomplex of $\mathcal{L}$ for any $\sigma \in \mathcal{K}$, and for any $\sigma_1, \sigma_2 \in \mathcal{L}$, $\Phi( \sigma_1 \cap \sigma_2) \subseteq \Phi(\sigma_1) \cap \Phi(\sigma_2)$.

We say that a carrier map $\Phi: \mathcal{K} \rightarrow 2^\mathcal{L}$
is \emph{rigid} if for every simplex $\sigma \in \mathcal{K}$ of dimension $d$, the subcomplex $\Phi(\sigma)$ is pure of dimension $d$. It is is \emph{strict} if for every simplices $\sigma, \tau \in \mathcal{K}$, $\Phi(\sigma \cap \tau) = \Phi(\sigma) \cap \Phi(\tau)$. Finally, it
carries a simplicial vertex map $\mu: \mathcal{K} \rightarrow \mathcal{L}$ if, for any $\sigma \in \mathcal{K}$, $\mu(\sigma) \in \Phi (\sigma)$.
\end{definition}

\begin{definition}[Star of a vertex]\label{def:absstar}
	Let $v \in V(\mathcal K)$. We define the star of $v$ as the subcomplex of $\mathcal{K}$ of all simplices that contain $v$.
\end{definition}

Since we are interested in relating combinatorial topology with it's point-set counterpart, we need a precise definition for topological spaces represented by abstract simplicial complexes. First we start with the geometric interpretation of a simplex.

\begin{definition}[Geometric simplex] \label{def:geosimp}
	Let $\mathcal{K}$ be an abstract simplicial complex, and $\sigma \in F(\mathcal{K})$.
	
	We define the geometric realization of $\sigma$, denoted by $| \sigma |$ as the set of affine functions from $\sigma$ into the closed interval $[0,1]$. That is $| \sigma | =  \{ f : \sigma \rightarrow [0,1] \; | \; \sum \limits_{v \in \sigma} f(v) = 1\}$. Elements of $| \sigma |$ are called points of $|\sigma|$.
	
	In order to make proofs more readable, we will also express the points of a geometric simplex in algebraic form. That is $\sum \limits_{v \in \sigma} f(v) \cdot v$.
\end{definition}

Intuitively, the affine functions form a coordinate system where the vertices in $\sigma$ are the generators. A $k$-dimensional geometric simplex is homeomorphic to a $k$-dimensional ball, and is embeddable into a $k$-dimensional Euclidean Space. Notice that this definition has the advantage that it is independent from embeddings.

We have defined the geometric realization of an individual simplex, however we would like to have a point-set topological space for the whole abstract simplicial complex.

\begin{definition}[Geometric Simplicial Complex]\label{def:geosimpcomp}
	Let $\mathcal{K}$ be an abstract simplicial complex, we define the geometric realization of $\mathcal{K}$, denoted by $|\mathcal{K}|$ as the quotient space $\coprod \limits _{\sigma \in F(\mathcal{K})} |\sigma| / R$. Where $\coprod \limits _{\sigma \in F(\mathcal{K})} |\sigma|$ is the disjoint union of all geometric simplices of $\mathcal{K}$, and $R$ is the equivalence relation given by $f \underset{R}{\sim} g$ iff $f^{-1}(0,1] = g^{-1}(0,1]$ and $f(v) = g(v)$ for all $v \in f^{-1}(0,1]$.
\end{definition}

In this definition we create disjoint geometric simplices and glue them along shared points. Notice that equivalence relation $R$ defines shared points as functions that have the same non-zero coordinates.

\begin{definition}[Geometric Star of a vertex]\label{def:star}
Let $v \in V(\mathcal{K})$ be a vertex of an abstract simplicial complex $\mathcal{K}$. We define the closed star of $v$, $\cstar(v)$ as the closed subset of $ \vert \mathcal{K} \vert$ induced by the geometric realization of the simplices that contain $v$. More precisely, $\cstar(v) = \bigcup \limits _{v \in \sigma } \vsigma$.
The open star of a vertex is the interior of the closed star, and denoted by $\ostar(v) = \interior(\cstar(v))$; note that $\interior(v)=v$ for every vertex. Unless explicitly stated, we will refer to the closed star of a vertex $v$ when using $\cstar(v)$.
\end{definition}


Carrier maps are used to specify the validity conditions of a task. A simplex in the input complex $\mathcal{I}$, which corresponds to a valid initial configuration, is mapped to a subcomplex of the output complex $\mathcal{O}$. This subcomplex corresponds to the valid different outputs that are allowed for this input. 

Notice that any chromatic subdivision $\textrm{Sub}(\mathcal{I})$ of a chromatic simplicial complex $\mathcal{I}$ induces a carrier map $\Phi: \mathcal{I} \rightarrow \textrm{Sub}(\mathcal{I})$. $\Phi$ maps each simplex $\sigma$ into a simplicial complex $\textrm{Sub}(\sigma)$. 



The following definition gives the standard meaning of the carrier $\textrm{carr}(\tau, \Phi)$
of a simplex $\tau \in \mathcal{O}$ for a strict carrier map $\Phi: \mathcal{I} \rightarrow 2^{\mathcal{O}}$:

\begin{definition}\label{def:carrcomp}
 Let $ \mathcal{I} , \mathcal{O}$ be finite simplicial complexes and $\Phi : \mathcal{I} \rightarrow 2^{\mathcal{O}}$ be a strict carrier map. For each simplex $\tau \in \Phi(\mathcal{I})$, there exists a unique simplex $\sigma \in \mathcal{I}$ of smallest dimension, such that $\tau \in \Phi(\sigma)$. We say that this $\sigma$ is the carrier of $\tau$ under $\Phi$, denoted $\textrm{carr}(\tau, \Phi)$.
\end{definition}

